SnapFuzz: An Efficient Fuzzing Framework for Network Applications

In recent years, fuzz testing has benefited from increased computational power and important algorithmic advances, leading to systems that have discovered many critical bugs and vulnerabilities in production software. Despite these successes, not all applications can be fuzzed efficiently. In particular, stateful applications such as network protocol implementations are constrained by their low fuzzing throughput and the need to develop fuzzing harnesses that reset their state and isolate their side effects. In this paper, we present SnapFuzz, a novel fuzzing framework for network applications. SnapFuzz offers a robust architecture that transforms slow asynchronous network communication into fast synchronous communication, snapshots the target at the latest point at which it is safe to do so, speeds up all file operations by redirecting them to a custom in-memory filesystem, and removes the need for many fragile modifications, such as configuring time delays or writing clean-up scripts, together with several other improvements. Using SnapFuzz, we fuzzed five popular networking applications: LightFTP, TinyDTLS, Dnsmasq, LIVE555 and Dcmqrscp. We report impressive performance speedups of 62.8x, 41.2x, 30.6x, 24.6x, and 8.4x, respectively, with significantly simpler fuzzing harnesses in all cases. Through its performance advantage, SnapFuzz has also found 12 extra crashes compared to AFLNet in these applications.

==> design-impl.tex <==
\snapfuzz has two main goals: significantly increase fuzzing throughput, and simplify the  construction of fuzzing harnesses.

At a high-level, \snapfuzz accomplishes these goals by intercepting all the communication between the target application and its environment via binary rewriting (\S\ref{sec:binary-rewriting}).
By controlling this communication, \snapfuzz can then:
\begin{enumerate}

      \item Redirect all file operations to use an in-memory filesystem (\S\ref{sec:in-mem-fs}).
            This improves the performance of these operations, and obviates the need for user-provided clean-up scripts, as \snapfuzz can automatically clean up after each fuzzing iteration by simply discarding the in-memory state.

      \item Replace internet sockets by UNIX domain sockets, which improves performance, as UNIX domain sockets are faster (\S\ref{sec:domain-sockets}).

      \item Notify the fuzzer when the target application is ready to accept a new
            request or when a response is ready to be consumed (\S\ref{sec:snapfuzz-protocol}).
            This eliminates all the custom delays that users need to insert in order to synchronise the communication between the fuzzer and the target application.
            This improves fuzzing throughput and also makes it easier to write fuzzing harnesses, as users don't need to worry about these delays anymore.

      \item Eliminate custom delays, unnecessary system calls and potentially expensive clean-up routines that are part of the target application (\S\ref{sec:eliminate-delays}).
            This improves the fuzzing throughput, with the only downside of missing bugs in the clean-up routines themselves. 

      \item Automatically defer the forkserver to the latest point at which it is safe to start it (\S\ref{sec:deferred-forkserver}).
            This eliminates the need for manual annotations and achieves the best possible performance.

      \item Propagate signals from child processes (\S\ref{sec:signals}).
            This ensures no crashes are missed during fuzzing.

      \item Pin threads and processes to available CPUs (\S\ref{sec:pinning}).
            This improves performance, without the need for any user intervention.

\end{enumerate}

\snapfuzz is implemented on top of \aflnet, and targets the Linux platform.
As such, it makes use of various OS facilities provided by Linux.
However, \snapfuzz could in principle be implemented on other platforms too.

\subsection{Binary Rewriting}
\label{sec:binary-rewriting}

\snapfuzz implements a load-time binary rewriting subsystem that dynamically
intercepts both the loader's and the target's functionalities in order to monitor and modify all external behaviours of the target application.

Applications interact with the external world via \emph{system calls}, such as \code{read()} and \code{write()} in Linux, which provide various OS services.
As an optimization, Linux provides some services via \emph{vDSO (virtual Dynamic Shared Object)} calls.  vDSO is essentially a small shared library injected by the kernel in every application in order to provide fast access to some services.  For instance, \emph{gettimeofday()} is typically using a vDSO call on Linux. 

The main goal of the binary rewriting component of \snapfuzz is to intercept all the system calls and vDSO calls issued by the application being fuzzed, and redirect them to a \emph{system call handler}.  The rest of this subsection presents how this interception is realised and can be skipped by readers less interested in the technical details involved. 

Binary rewriting in \snapfuzz employs two major components:
1)~the rewriter module, which scans the code for specific functions, vDSO and system call assembly opcodes, and redirects them to the plugin module, and
2)~the plugin module where \snapfuzz resides.

\subsubsection{Rewriter}
\label{subsec:rewriter}

\snapfuzz is an ordinary dynamically linked executable that is provided with a path to a target application together with the arguments to invoke it with.
When \snapfuzz is launched, the expected sequence of events of a standard Linux operating system are taking place, with the first step being the dynamic loader that loads \snapfuzz and its dependencies in memory.

%
%
%

When \snapfuzz starts executing, it inspects the target's ELF binary to obtain information about its interpreter, which in our implementation is always the standard Linux \textit{ld} loader.

\snapfuzz then scans the loader code for system call assembly opcodes and some special functions in order to instruct the loader to load the \snapfuzz plugin.
%
In particular, the rewriter:
(1)~intercepts the dynamic scanning of the loader in order to append the \snapfuzz plugin shared object as a dependency, and
(2)~intercepts the initialisation order of the shared libraries in order to prepend the \snapfuzz plugin initialisation code (in the \textit{.preinit\_array}).

%

After the \snapfuzz rewriter finishes rewriting the loader, execution is passed to the rewritten loader in order to load the target application and its library dependencies.
At this stage, all system calls and some specific loader functions are monitored.
As the normal execution of the loader progresses, \snapfuzz intercepts its \code{mmap} system calls used to load libraries into memory, and scans these libraries in order to recursively rewrite their system calls and redirect them to the \snapfuzz plugin.
The \snapfuzz rewriter is based on the open-source load-time binary rewriter SaBRe~\cite{sabre}.

\subsubsection{Plugin}

The \snapfuzz plugin implements a simple API that exposes three important functions:
(1)~An initialisation function that will be the first code to run after loading is done (this function is prepended dynamically to the \textit{.preinit\_array} of our target's ELF binary),
(2)~a function to which all system calls will be redirected, which we call the \textit{system call handler}, and
(3)~a similar function to which all vDSO calls will be redirected, the \textit{vDSO handler}.

After the loader completes, execution is passed to the target application, which will start by executing \snapfuzz's initialisation function.
Per the ELF specification, execution starts from the function pointers of \textit{.preinit\_array}.
This is a common ELF feature used by LLVM sanitizers to initialise various internal data structures early, such as the shadow memory~\cite{ASan,MSan}.
\snapfuzz is using the same mechanism to initialise its subsystems like its in-memory filesystem before the execution starts.

After the initialisation phase of the plugin, control is passed back to the target application and normal execution is resumed.
At this stage, the \snapfuzz plugin is only executed when the target is about to issue a system call or a vDSO call.
When this happens, the plugin checks if the call should be intercepted, and if so, it further redirects it to the appropriate handlers, after which control is returned back to the target.

The \snapfuzz plugin is also responsible to handle and guard against recursive calls and vDSO.
For example, the plugin itself is allowed to issue system calls through the use of the target's \textit{libc}.
To achieve this, \snapfuzz's plugin is guarding every jump from the target application to the plugin with a thread local flag.

%

%
%
%

\subsection{In-memory filesystem}
\label{sec:in-mem-fs}

As mentioned before, \snapfuzz redirects all file operations to use a custom in-memory filesystem.
This reduces the overhead of reading and writing from a storage medium, and eliminates the need for manually-written clean-up scripts to be run after each fuzzing operation, as the clean-up can be done automatically by simply discarding the in-memory state.

%
%

\snapfuzz implements a lightweight in-memory filesystem, which uses two distinct mechanisms, one for files and the other for directories.

For files, \snapfuzz's in-memory filesystem uses the recent \break \code{memfd\_create()} system call, introduced in Linux in 2015~\cite{memfd_create}.
This system call creates an anonymous file and returns a file descriptor that refers to it.
The file behaves like a regular file, but lives in memory.

Under this scheme, \snapfuzz only needs to specially handle system calls that initiate interactions with a file through a pathname (like the \code{open} and \code{mmap} system calls).
All other system calls that handle file descriptors are compatible by default with the file descriptors returned by \code{memfd\_create}.

When a target application opens a file, the default behavior of \snapfuzz is to
check if this file is a regular file (e.g. device files are ignored), and if
so, create an in-memory file descriptor and copy the whole contents
of the file in the memory address space of the target application through the
memory file descriptor.
\snapfuzz keeps track of pathnames in order to avoid reloading the same file twice. This is not only a performance optimization but also a correctness requirement, as the application might have changed the contents of the file in memory.

%
%

Implementing an in-memory filesystem from scratch with anonymous mapping through \textit{mmap} and rewriting all I/O system calls to become function calls operating on the in-memory files would be even more efficient than the current \snapfuzz implementation which is still issuing regular system calls and thus paying the associated context-switch overhead.
%
But developing such a subsystem that is compatible with the large diversity of system call options available on Linux is a laborious and difficult task, which is why we have opted for a \code{memfd\_create}-based approach.

For directories, \snapfuzz takes advantage of the \textit{Libsqlfs} library~\cite{libsqlfs}, which implements a POSIX-style file system on top of the SQLite database and allows applications to have access to a full read/write filesystem with its own file and directory hierarchy.
\textit{Libsqlfs} simplifies the emulation of a real filesystem with directories and permissions.
\snapfuzz uses \textit{Libsqlfs} for directories only, as we observed better performance for files via \textit{memfd\_create}.
%

With the in-memory filesystem in-place, \snapfuzz can already implement two important optimizations: a smart deferred forkserver (\S\ref{sec:deferred-forkserver}) and an efficient state reset (\S\ref{sec:state-reset}).

\subsection{Smart deferred forkserver}
\label{sec:deferred-forkserver}

As discussed in \S\ref{sec:afl}, the deferred forkserver can offer great performance benefits by avoiding initialisation overheads in the target.
Such overheads include loading the shared libraries of a binary, parsing configuration files and cryptographic initialisation routines.
Unfortunately, for the deferred forkserver to be used, the user needs to manually modify to source code of the target.
Furthermore, the deferred forkserver cannot be used after the target has created threads, child processes, temporary files, network sockets, offset-sensitive file descriptors, or shared-state resources, so the user has to carefully decide where to place it: do it too early and optimisation opportunities are missed, do it too late and correctness is affected.
%

%
%

\snapfuzz makes two important improvements to the deferred forkserver: first, it makes it possible to defer it much further than usually possible with \afl's architecture, and second, it does so automatically, without any need for manual source modifications.  This is made possible through \snapfuzz's binary rewriting mechanism together with its in-memory filesystem and custom network communication mechanism.

There are two reasons for which \snapfuzz can place the forkserver after many system calls which normally would have caused problems: (1)~its use of an in-memory filesystem in the case of file operations, as it transforms external side effects into in-memory changes;
and (2)~its custom network communication mechanism which allows it to skip network setup calls such as \code{socket} and \code{accept} (see \S\ref{sec:domain-sockets}).

Via binary rewriting, \snapfuzz intercepts each system call, and places the forkserver just before it encounters either a system call that spawns new threads (\code{clone}, \code{fork}), or one used to receive input from a client.

%
%

%
%
%
%
%
%
%
%

%
%

The reason \snapfuzz still has to stop before the application spawns new threads is that the forkserver relies on \code{fork} to spawn new instances to be fuzzed, and \code{fork} cannot reconstruct existing threads---in Linux, forking a multi-threaded application creates a process with a single thread~\cite{fork}.
As a possible mitigation, we tried to combine \snapfuzz and the \textit{pthsem / GNU pth} library~\cite{pthsem}---a green threading library that provides non-preemptive priority-based scheduling, with the green threads executing inside an event-driven framework---but the performance overhead was too high.
%

In particular, we used \textit{pthsem} with \lightftp, as this application has to execute two \code{clone} system calls before it accepts input.
With \textit{pthsem} support, \snapfuzz's forkserver can skip these two \code{clone} calls, as well as 37 additional system calls, as now \snapfuzz can place the forkserver just before \lightftp is ready to accept input.
However, despite this gain, the overall performance was 10\% lower than in the version of \snapfuzz without \textit{pthsem}, due to the overhead of this library.
%
Ideally, \snapfuzz should implement a lightweight thread reconstruction mechanism to recreate all dead threads, but this is left as future work.

%

%
%
%

%
%

%
%
%

%
%

%

%

%

%

%

%

\subsection{Efficient state reset}
\label{sec:state-reset}

%
%
%
%

To use \aflnet, users typically have to write a clean-up script to reset the application state after each iteration.
For instance, \lightftp under \aflnet requires a Bash script to be invoked in every iteration in order to clean up any directories or files that have been created in the previous iteration.
Under \snapfuzz, there is no need for such a cleanup script, which simplifies the test harness construction, and improves performance by avoiding the invocation of the cleanup script.

In the simplest case where \afl checkpoints the target application before \code{main}, no filesystem modifications have happened at the point where the forkserver is placed.
So when a fuzzing iteration has finished, the target application process just exits and the OS discards its memory, which includes any in-memory filesystem modifications made during fuzzing.
Then, when the forkserver spawns a new instance of the target application, the filesystem is brought back to a state where all initial files of the actual filesystem are unmodified.

The situation is more complicated when the deferred forkserver is placed after the target application has already created some files.
When the forkserver creates a new instance to be fuzzed, the Linux kernel shares the memory pages associated with the newly-created in-memory files between the new instance and the forkserver.
%
%
%
This is problematic for \snapfuzz, as now any modifications to the in-memory files by the fuzzed application instance will persist even after the instance finishes execution.
%
So in the next iteration, when the forkserver creates a new instance, this new instance will inherit those modifications too.

\snapfuzz solves this issue as follows. 
First, note that \snapfuzz knows whether the application is executing before or after the forkserver's checkpoint, as it intercepts all system calls, including \code{fork}.
%
While the target application executes before the forkserver's checkpoint, \snapfuzz allows all file interactions to be handled normally. 
When a new instance is requested from the forkserver, \snapfuzz recreates in the new instance all in-memory files registered in the in-memory filesystem and copies all their contents by using the efficient \code{sendfile} system call once per in-memory file.

\subsection{UNIX domain sockets}
\label{sec:domain-sockets}

\aflnet uses the standard Internet sockets (TPC/IP and UDP/IP) to communicate to the target and send it fuzzed inputs.
The Internet socket stack includes functionality---such as calculating checksums of packets, inserting headers, routing---which is unnecessary when fuzzing applications on a single machine.

%

%

To eliminate this overhead, \snapfuzz replaces Internet sockets with UNIX domain sockets.
More specifically, \snapfuzz uses Sequenced Packets sockets (\code{SOCK\_SEQPACKET}).
This configuration offers performance benefits and also simplifies the implementation.
Sequenced Packets are quite similar to TCP, providing a sequenced, reliable, two-way connection-based data transmission path for datagrams.
The difference is that Sequenced Packets require the consumer (in our case the \snapfuzz plugin running inside the target application) to read an entire packet with each input system call.
This atomicity of network communications simplifies corner cases where the target application might read only parts of the fuzzer's input due to scheduling or other delays.
By contrast, \aflnet handles this issue by exposing manually defined knobs for introducing delays between network communications.

%
Our modified version of \aflnet creates a socketpair of UNIX domain sockets with the Sequenced Packets type, and passes one end to the forkserver, which later passes it to the \snapfuzz plugin.
The \snapfuzz plugin initiates a handshake with the modified \aflnet, after which \aflnet is ready to submit generated inputs to the target or consume responses.

Translating networking communications from Internet sockets to UNIX domain sockets is not trivial, as \snapfuzz needs to support the two main IP families of TCP and UDP which have a slightly different approach to how network communication is established.
In addition, \snapfuzz also needs to support the different synchronous and asynchronous network communication system calls like \code{poll}, \code{epoll} and \code{select}.

For the TCP family, the \code{socket} system call creates a TCP/IP socket and returns a file descriptor which is then passed to \code{bind}, \code{listen} and finally to \code{accept}, before the system is ready to send or receive any data.
\snapfuzz monitors this sequence of events on the target and when the \code{accept} system call is detected, it returns the UNIX domain socket file descriptor from the forkserver.
\snapfuzz doesn't interfere with the \code{socket} system call and intentionally allows its normal execution in order to avoid complications with target applications that perform advanced configurations on the base socket.
This strategy is similar to the one used by the in-memory file system via the \code{memfd\_create} system call (\S\ref{sec:in-mem-fs}) in order to provide compatibility by default.

The UDP family is handled in a similar way, with the only difference that instead of monitoring for an \code{accept} system call to return the UNIX domain socket of the forkserver, \snapfuzz is monitoring for a \code{bind} system call.

\snapfuzz also needs to handle asynchronous networking communications as the base socket will not receive any prompt for incoming connections.
%
\snapfuzz intercepts all asynchronous system calls and the first time the base socket is passed to an asynchronous system call like \code{poll}, it sets its state to be notified.
%
This informs the target application that an incoming connection is waiting to be handled, making it progress to execute an \code{accept} system call.

In summary, \snapfuzz's use of UNIX domain sockets provides two key advantages: it simplifies the construction of test harnesses, which don't need to specify fragile delays between network communications anymore; and speeds up fuzzing by eliminating these delays and the unnecessary overhead of Internet sockets.

%

%
\subsection{Eliminating protocol-related delays}
\label{sec:snapfuzz-protocol}

\begin{figure}
      \centering
      \resizebox{1.00\columnwidth}{!}{
            \includegraphics{imgs/snapfuzz-prot.pdf}
      }
      \caption{Messages exchanged for each \texttt{recv} and \texttt{send}.}
      \captionsetup{justification=centering}
      \label{fig:sf-prot}
\end{figure}

Network applications often implement multistep protocols with multiple requests and replies per session.
One of \aflnet's main contributions is to infer the network protocol starting from a set of recorded message exchanges.
However, \aflnet cannot guarantee that during a certain fuzzing iteration the target will indeed respect the protocol.
Deviations might be possible for instance due to a partly-incorrect protocol being inferred, bugs in the target application, or most commonly due to the target not being ready to send or receive a certain message.

Therefore, \aflnet performs several checks and adds several user-specified delays  to ensure communication is in sync with the protocol.
These protocol-related delays, which can significantly degrade the fuzzing throughput, are:

%
%
%
%
\begin{enumerate}
      \item A delay to allow the server to initialise before \aflnet attempts to communicate.
      \item A delay specifying how long to wait before concluding that no responses are forthcoming and instead try to send more information, and
      \item A delay specifying how long to wait after each packet is sent or received.
\end{enumerate}

These delays are necessary, as otherwise the Linux kernel will reject packets that come too fast while the target is not ready, and \aflnet will desynchronize from its state machine.
But they cause a lot of time to be wasted, essentially because \aflnet does not know whether the target is ready to send or receive information.
%

\snapfuzz overcomes this challenge by notifying \aflnet about the next action of the target.
It does this by introducing a second UNIX domain socket, namely the \textit{control socket}, which is used as a send-only channel from the \snapfuzz plugin to \aflnet to inform  the latter if the target will next execute a \code{recv} or a \code{send} system call, as shown in Figure~\ref{fig:sf-prot}. 
%

%
In summary, \snapfuzz makes it possible to remove three important communication delays, which simplifies fuzzing harnesses and leads to significant performance gains, as we will show in the evaluation.

\subsection{Additional optimizations}
\label{sec:extras}

In this section, we discuss several additional optimizations performed by \snapfuzz.
%
%
They concern developer-added delays, writes to \code{stdout/stderr}, signal propagation, server termination and thread pinning, and highlight the versatility of \snapfuzz's approach in addressing a variety of challenges and inefficiencies when fuzzing network applications.
%

\subsubsection{Eliminating developer-added delays}
\label{sec:eliminate-delays}

Occasionally, network applications add sleeps or timeouts in order to avoid high CPU utilisation when they poll for new connections or data.
\snapfuzz removes these delays, making those calls use a more aggressive polling model.

We also noticed that in some cases application developers deliberately choose to add sleeps in order to wait for various events.
For example, \lightftp adds a one second sleep in order to wait for all its threads to terminate.
This might be fine in a production environment, but during a fuzzing campaign such a delay is unnecessary and expensive.
\snapfuzz completely skips such sleeps by intercepting and then not issuing this family of system calls at all.

\subsubsection{Avoiding \code{stdout/stderr} writes}

By default, \afl redirects \code{stdout} and \code{stderr} to \code{/dev/null}.
This is much more performant than actually writing to a file or any other medium, as the kernel optimizes those operations aggressively.
\snapfuzz goes one step further and saves additional time by completely skipping any system call that targets \code{stdout} or \code{stderr}. 

\subsubsection{Signal Propagation}
\label{sec:signals}

Some applications use a multi-process rather than a multi-threaded concurrency model.
In this case, if a subprocess crashes with a segfault, the signal might not be propagated properly to the forkserver and the crash missed.
We stumbled upon this case with the \dcmqrscp server (\S\ref{sec:dcmqrscp}) where a valid new bug was manifesting, but \aflnet was unable to detect the issue as the main process of \dcmqrscp never checked the exit status of its child processes.

As \snapfuzz has full control of the system calls of the target, whenever a process is about to exit, it checks the exit status of its child processes too.
If an error is detected, it is raised to the forkserver.

\subsubsection{Efficient server exit}

Network servers usually run in a loop.
This loop is terminated either via a special protocol-specific keyword or an OS signal.
Since \aflnet cannot guarantee that each fuzzing iteration will finish via a termination keyword, if the target does not terminate, it sends it a \code{SIGTERM} signal and waits for it to terminate.

Signal delivery is slow and also servers might take a long time to properly terminate execution.
In the context of fuzzing, proper termination is not so important, while fuzzing throughput is.
\snapfuzz implements a simple mechanism to terminate the server: when it receives an empty string, this signals that the fuzzer has no more inputs to provide and the application is instantly killed.
This obviously has the downside that it could miss bugs in the termination routines, but these could be tested separately.
%
%

\subsubsection{Smart affinity}
\label{sec:pinning}

\afl assumes that its targets are single-threaded and thus tries to pin the fuzzer and the target to two free CPUs.
Unfortunately, there is no mechanism to handle multi-threaded applications, other than just turning off \afl's pinning mechanism.
\snapfuzz can detect when a new thread or process is about to be spawned as both \code{clone} and \code{fork} system calls are intercepted.
This creates the opportunity for \snapfuzz to take control of thread scheduling by pinning threads and processes to available CPUs.
\snapfuzz implements a very simple algorithm that pins every newly created thread or process to the next available CPU.



